Lecture Notes on Free Probability

These lecture notes provide an introduction to free probability theory, with a focus on tools and techniques useful in the study of large random matrices. Topics include freeness, free cumulants, additive and multiplicative free convolution, the R- and S-transforms, subordination theory, and operator-valued extensions. Applications to asymptotic freeness and linearization methods are discussed in detail. The notes aim to be accessible to graduate students with a background in functional analysis and probability. The lecture notes were originally written for a graduate course. They are updated to include recent results on subordination and linearization methods in free probability.

==> mathPreambuleReport.tex <==
%\documentclass[12pt]{amsart}

\usepackage{amssymb, amsfonts, amsmath, amsthm}
%\usepackage{enumerate} %-- this is simpler package
\usepackage{enumitem} %-- this gives a bit more freedom
\usepackage{times}
\usepackage{yfonts}
\usepackage{egothic}
\usepackage[T2A,T1]{fontenc}
%\usepackage{fontspec}

\usepackage{mathdots}

\usepackage[russian, english]{babel}
\usepackage[dvipsnames]{xcolor}
\usepackage{wrapfig}

\input Rothdn.fd
\renewcommand*\initfamily{\usefont{U}{Rothdn}{xl}{n}}

\usepackage{bbm}
\newcommand{\1}{\mathbbm{1}} % Blackboard bold 1 for indicator function.


\RequirePackage{graphicx}
\RequirePackage{hyperref}
\RequirePackage[small,bf]{caption}
\RequirePackage{actuarialangle}

\usepackage{tikz}

%%%%%%%%%%%%%%%%%%%%%
%Add nice headers
%%%%%%%%%%%%%%%%%%

%\usepackage{fancyhdr}
%\fancyfoot{}
%\fancyhead[RO,LE]{\thepage}
%\fancyhead[LO]{\leftmark}
%\fancyhead[RE]{\rightmark}
%\renewcommand{\headheight}{14pt}

%\renewcommand{\baselinestretch}{1.2}
\renewcommand{\emph}{\textbf}

%\usepackage[a4paper, left = 4cm, right = 4cm, top=3cm, bottom=4cm]{geometry}
%\setlength{\marginparwidth}{3.8cm}
%%%%%%%%%%%%%%%%%%%%%%
%Modify Table of Contents
%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{titletoc}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Define format of sections, subsections and subsubsections
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{titlesec}
%\titleformat{\section}[frame] 
%{\normalfont}
%{\filright
%\footnotesize
%$\heartsuit$
%     \enspace SECTION \thesection\enspace}
%{8pt}
%{\LARGE\frakfamily\filcenter}
%
%\titleformat{\subsubsection}
%{\normalfont\normalsize\bfseries}
%{\thesubsubsection}
%{1em}
%{}
%
%\titleformat{\subsection}[display] 
%{\normalfont\fillast}
%{\Large\frakfamily section \oldstylenums{\thesubsection}} 
%{1ex minus .1ex}
%{\Large\egothfamily}
%
%\titlespacing{\section} {3pc}{*3}{*2}[3pc]
%\titlespacing{\subsection} {3pc}{*3}{*2}[3pc]


%%%%%%%%%
%%Ivrit letters
%%
%%%%%%%%%%%%%%
%\DeclareFontFamily{U}{rcjhbltx}{}
%\DeclareFontShape{U}{rcjhbltx}{m}{n}{<->rcjhbltx}{}
%\DeclareSymbolFont{hebrewletters}{U}{rcjhbltx}{m}{n}

%% remove the definitions from amssymb
%\let\aleph\relax\let\beth\relax
%\let\gimel\relax\let\daleth\relax
%
%\DeclareMathSymbol{\aleph}{\mathord}{hebrewletters}{39}
%\DeclareMathSymbol{\beth}{\mathord}{hebrewletters}{98}\let\bet\beth
%\DeclareMathSymbol{\gimel}{\mathord}{hebrewletters}{103}
%\DeclareMathSymbol{\daleth}{\mathord}{hebrewletters}{100}\let\dalet\daleth
%
%\DeclareMathSymbol{\lamed}{\mathord}{hebrewletters}{108}
%\DeclareMathSymbol{\mem}{\mathord}{hebrewletters}{109}\let\mim\mem
%\DeclareMathSymbol{\ayin}{\mathord}{hebrewletters}{96}
%\DeclareMathSymbol{\tsadi}{\mathord}{hebrewletters}{118}
%\DeclareMathSymbol{\qof}{\mathord}{hebrewletters}{114}
%\DeclareMathSymbol{\shin}{\mathord}{hebrewletters}{152}


%\renewcommand{\daleth}{\text{?}}
%\DeclareMathSymbol{\shin}{\text{?}}
\DeclareSymbolFont{cyrillic}{T2A}{cmr}{m}{n}
\DeclareMathSymbol{\zhe}{\mathalpha}{cyrillic}{198}
\DeclareMathSymbol{\sha}{\mathalpha}{cyrillic}{216}

%%%%%%%%%%%
%A shortcut for alignment environment and for equations
%%%%%%%%%%%
\newcommand{\bal}[1]{\begin{align*}#1\end{align*}}
\newcommand{\beq}[1]{\begin{equation}#1\end{equation}}

%A shortcut for matrices
\newcommand{\bmatr}[1]{\begin{bmatrix}#1\end{bmatrix}}


%%%colors
\newcommand{\blue}{\color{blue}}
\newcommand{\red}{\color{red}}
\newcommand{\orange}{\color{orange}}
\newcommand{\cyan}{\color{cyan}}
%\newcommand{\red}{\color{red}}
\newcommand{\magenta}{\color{magenta}}
\newcommand{\green}{\color{green}}


\newcommand{\bi}{\mathbf{i}} %quaternion units
\newcommand{\bj}{\mathbf{j}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\Z}{\mathbb{Z}} %ring of integers
\newcommand{\N}{\mathbb{N}} %natural numbers
\newcommand{\R}{\mathbb{R}}
\newcommand{\bC}{\mathbb{C}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\bS}{\mathbb{S}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\bH}{\mathbb{H}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\Corr}{\mathrm{Corr}}
\newcommand{\bP}{\mathbb{P}}
\renewcommand{\P}{\bP} %another version of probability
\newcommand{\Wg}{\mathrm{Wg}}
\newcommand{\Var}{\mathbb{V}\mathrm{ar}}
\newcommand{\Ad}{\mathrm{Ad}}
\newcommand{\Trace}{\mathrm{Tr}}
\newcommand{\eps}{\varepsilon}
\renewcommand{\phi}{\varphi}
\renewcommand{\Re}{\mathrm{Re}\,} %redefining Re and Im commands
\renewcommand{\Im}{\mathrm{Im}\,}


\newcommand{\df}{\stackrel{{{\mathrm{def}}}}{=}}
\newcommand{\func}[1]{\mathrm{#1}}
\newcommand\stack[2]{\genfrac{[}{]}{0pt}{}{#1}{#2}}
\newcommand{\QED}{\hfill $\square$}  

\newcommand{\scP}[2]{\left\langle #1, #2\right\rangle} %scalar product
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}


\newcommand{\ovln}[1]{\overline{#1}}
\newcommand{\wh}{\widehat}
\newcommand{\wt}{\widetilde}
\newcommand{\oc}[1]{\overset{\circ}{#1}} %Puts a circle on the argument. 

\newcommand{\Cl}{\mathcal{C}\ell}
\newcommand{\rn}{\mathrm{rn}}
\DeclareMathOperator{\blk}{bk} %number of blocks in a partition
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\ord}{ord} %order of a function
\DeclareMathOperator{\supp}{supp} %support of a measure
\DeclareMathOperator{\diag}{diag} %diagonal matrix
\DeclareMathOperator{\Id}{Id}


%%%%%%%%%%%%%%%%%%%%%%%%%%
%Various shortcuts for convergences
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\pwcv{\stackrel{\scriptscriptstyle p.w.}{\longrightarrow}}     % pointwize convergence
\def\ascv{\stackrel{\scriptscriptstyle a.s.}{\longrightarrow}}     % almost sure convergence
\def\pcv{\stackrel{\scriptscriptstyle \P}{\longrightarrow}}        % convergence in P
\def\ltcv{\stackrel{\scriptscriptstyle\LL^2}{\longrightarrow}}      % L2 convergnece
\def\lpcv{\stackrel{\scriptscriptstyle\LL^p}{\longrightarrow}}      % Lp convergnece
\def\dcv{\stackrel{\scriptscriptstyle d}{\longrightarrow}}         % convergence in d
\def\wcv{\stackrel{\scriptscriptstyle w}{\longrightarrow}}         % weak
\def\deq{\stackrel{\scriptscriptstyle d}{=}}			   % equal in d
\def\toinf{\to \infty}
\def\ci{\perp\!\!\!\perp}  % conditional independence
\newcommand{\convpoint}{\stackrel{p.w.}{\longrightarrow}}
\newcommand{\conv}{\rightarrow}
\newcommand{\xto}{\xrightarrow}
\newcommand{\dashfrom}{\dashleftarrow}
\newcommand{\dashto}{\dashrightarrow}
\def\pto{\stackrel{p}{\longrightarrow}} %convergence in probability


%\newcommand{\B}{\BB} %another version for Borel field
\newcommand{\fL}{\mathrm{L}}   %upright L for functional spaces
\newcommand{\XX}{\mathcal{X}} %Determinantal field
\newcommand{\bT}{\mathbb{T}} %Torus
\newcommand{\TT}{\mathcal{T}} %Graph of tilings
\newcommand{\calS}{\mathcal{S}}
\newcommand{\RR}{\mathcal{R}} %Another form of R-transform.
\newcommand{\MM}{\mathcal{M}} %right module of quaternion polynomials
\newcommand{\VV}{\mathcal{V}} %standard left module for Temperley-Lieb algebra.
\newcommand{\LL}{\mathcal{L}} %Normalized bracket polynomial
\newcommand{\KK}{\mathcal{K}} %rescaled kernel
\newcommand{\II}{\mathcal{I}} %interface, or interval
\newcommand{\HH}{\mathcal{H}} %sigma-field 
\newcommand{\GG}{\mathcal{G}} %another sigma-field 
\newcommand{\FF}{\mathcal F}
\newcommand{\DD}{\mathcal D}
\newcommand{\CC}{\mathcal C}
\newcommand{\BB}{\mathcal B}
\renewcommand{\AA}{\mathcal A}

\newcommand{\PP}{\mathcal P} %poset
\newcommand{\pp}{\mbox{\egothfamily p}}

\newcommand{\ac}[1]{\actuarialangle{#1}}




%\declaretheoremstyle[headfont=\normalfont\bfseries, 
%postheadspace=\newline, bodyfont=\itshape, spaceabove=0.5cm,
%spacebelow=0.5cm, notebraces=< >, shaded={bgcolor={blue!15!gray!5}}]{myLemmaStyle}

%\declaretheoremstyle[headfont=\normalfont\bfseries, 
%postheadspace=\newline, bodyfont=\itshape, spaceabove=0.5cm,
%spacebelow=0.5cm, notebraces=| |, shaded={bgcolor={yellow!20}}]{myThmStyle}

%\declaretheoremstyle[headfont=\large\egothfamily, 
%postheadspace=\newline, bodyfont=\itshape, spaceabove=0.5cm,
%spacebelow=0.5cm, notebraces=| |, shaded={bgcolor={yellow!20}}]{myThmStyle}



%\declaretheoremstyle[headfont=\normalfont\bfseries, 
%postheadspace=\newline, bodyfont=\itshape, spaceabove=0.5cm,
%spacebelow=0.5cm, notebraces=< >, shaded={bgcolor={Lavender!10}}]{myThmStyle}

%\declaretheorem[heading=Theorem, parent = section, style= myThmStyle]{theo}
%\declaretheorem[heading=Property, parent = section, style= myThmStyle]{pro}
%%\declaretheorem[thmbox = M]{theo}
%\declaretheorem[heading=Lemma, sibling=theo, style= myLemmaStyle]{lemma}
%\declaretheorem[heading=Corollary, sibling=theo, style= myLemmaStyle]{coro}
%\declaretheorem[heading=Example, sibling=theo, style= myLemmaStyle]{exa}

\theoremstyle{plain}
\newtheorem{theo}{Theorem}[section]
\newtheorem{lemma}[theo]{Lemma}
\newtheorem{propo}[theo]{Proposition}
\newtheorem{coro}[theo]{Corollary}


\theoremstyle{definition}
\newtheorem{defi}[theo]{Definition}
\newtheorem{conjecture}[theo]{Conjecture}
\newtheorem{claim}[theo]{Claim}
\newtheorem{problem}[theo]{Problem}

\theoremstyle{remark}
\newtheorem{remark}[theo]{Remark}
\newtheorem{exa}[theo]{Example}
\newtheorem{exe}[theo]{Exercise}
\newtheorem{pro}[theo]{Property}
\newtheorem*{solu*}{Solution}



